Flexible Caching in Trie Joins

Traditional algorithms for multiway join computation are based on rewriting the order of joins and combining results of intermediate subqueries. Recently, several approaches have been proposed for algorithms that are "worst-case optimal" wherein all relations are scanned simultaneously. An example is Veldhuizen's Leapfrog Trie Join (LFTJ). An important advantage of LFTJ is its small memory footprint, due to the fact that intermediate results are full tuples that can be dumped immediately. However, since the algorithm does not store intermediate results, recurring joins must be reconstructed from the source relations, resulting in excessive memory traffic. In this paper, we address this problem by incorporating caches into LFTJ. We do so by adopting recent developments on join optimization, tying variable ordering to tree decomposition. While the traditional usage of tree decomposition computes the result for each bag in advance, our proposed approach incorporates caching directly into LFTJ and can dynamically adjust the size of the cache. Consequently, our solution balances memory usage and repeated computation, as confirmed by our experiments over SNAP datasets.

==> background.tex <==
\section{Background}
\iffalse
\subsection{Relational Data model \& Trie join}
%Relational data model organizes elements and define a standard on the relations between elements. A join query Q is defined by a set of atoms(Q) denoted by Q =...R.

\subsection{Trie Leapfrog}
% Move to introduction to all data that isn't relevant to algorithm
% Everything else need to be exact and general
We describe LFTJ algorithm. LFTJ implementation is based on data which is stored in data structures similar to B-trees. The LFTJ uses the unary leapfrog as a building block, which resembles to sort-merge join while simultaneously joins unary relations (references). To support relations of arity > 1, they use Trie iterators. Each relation A(x,y,z) is presented as a trie, with each tuple (x,y,z)eA corresponding to a unique path through the trie from root to leaf (Figure). Each trie consists of multiple levels, while each level corresponds to a join attribute. To run the triejoin a join attribute order must be set by the optimizer. Different attributes' orders might effect the performance of the join. After choosing and order, all tries are constructed coherent with the order, lower attributes will be higher in the trie. For each join attribute 'A', perform an unary leapfrog on the tries that contain 'A'. When a match is encountered, go to the next level on all these tries and continue to the next attribute in order. If no match was found, go up these tries and look for the next match on the previous attribute. A join match is returned when a match is found at the last join attribute. The algorithm ends when no more matches are found at the first attribute.

As mentioned before, LFTJ have a very small footprint, which holds the current locations of the trie iterators, and generates streaming results. When working on data with no skew, a rare case in the real world, this algorithm is optimal. When the data is skewed, LFTJ might do redundant calculations. For example, in the query Q=R(x,y),S(y,z),T(x,z) and order x<y<z. if y=\{\{y1\}X5,\{y2\}X1000\}, the trie of R will hold 100 repetitions of y2. Each time there is a match on (*,y2)eR, LFTJ will calculate the whole path from R to T. In our case, this can take up to 999 of redundant calculations of the whole path. Notice, that this is relevant to 'z', as well as any other join attribute that is not the first. An early join attribute might save more deep searches, but on the other hand, a late join attribute will be more frequent and might save on the quantity of searches. 
\fi
